Simple ReFlow: Improved Techniques for Fast Flow Models

Diffusion and flow-matching models achieve remarkable generative performance but at the cost of many sampling steps, this slows inference and limits applicability to time-critical tasks. The ReFlow procedure can accelerate sampling by straightening generation trajectories. However, ReFlow is an iterative procedure, typically requiring training on simulated data, and results in reduced sample quality. To mitigate sample deterioration, we examine the design space of ReFlow and highlight potential pitfalls in prior heuristic practices. We then propose seven improvements for training dynamics, learning and inference, which are verified with thorough ablation studies on CIFAR10 $32 \times 32$, AFHQv2 $64 \times 64$, and FFHQ $64 \times 64$. Combining all our techniques, we achieve state-of-the-art FID scores (without / with guidance, resp.) for fast generation via neural ODEs: $2.23$ / $1.98$ on CIFAR10, $2.30$ / $1.91$ on AFHQv2, $2.84$ / $2.67$ on FFHQ, and $3.49$ / $1.74$ on ImageNet-64, all with merely $9$ neural function evaluations.

==> sections/2_related_work.tex <==
\section{Related Works}
% \jt{mention ways to improve RF, sd3}

Efforts for accelerating diffusion-based generation can be divided roughly into three branches: learning faster ODEs, using faster ODE solvers, and distilling probability flow ODEs. Below, we give a brief discussion of recent progress in respective categories. 
% \bah{keep order the same as the order of paragraphs below}. 


\textbf{Rectified flows.}

\textbf{Faster ODEs via couplings.} Generally, ODEs with straight generative trajectories can be solved accurately with substantially fewer velocity evaluations than those with high-curvature trajectories \citep{numanalysis}. In fact, probability flow ODEs with perfectly straight trajectories can translate one distribution to another with a single Euler step. This has motivated works on learning optimal transport (OT) ODEs such as Rectified Flow (RF) \citep{liu2022rf,liu2022rfmp,lee2024rfpp} and OT Flow Matching \citep{tong2023cfm,pooladian2023mfm}, or learning ODEs which directly minimize trajectory curvature \citep{lee2023curvature}.

\textbf{Fast sampling.} One can use higher-order solvers which utilize higher order differentials of the ODE velocity to take large integration steps or reduce truncation error \citep{karras2022edm,dockhorn2022genie,lu2022dpmsolver,zhang2023deis}. While this approach is generally training-free, recent works \citep{zhou2024amed,kim2024dode} have incorporated trainable components which minimize truncation error to further accelerate sampling.

\textbf{Distillation and Consistency Models.} The goal of distillation is to compress multiple probability flow ODE steps of a teacher diffusion model into a single evaluation of a student model. Representative methods are progressive distillation \citep{salimans2022pd}, and consistency distillation \citep{song2023cm,song2024icm,kim2024ctm,geng2024ect}.

We also remark that faster ODEs have several practical benefits over other approaches. Since translation along an ODE is a bijective map, we can achieve fast inversion and likelihood evaluation by integrating the ODE backwards starting from data. Furthermore, faster ODEs can be combined with distillation or fast samplers to achieve a greater effect. For instance, \cite{lee2023curvature,liu2024instaflow,liu2024slimflow} have observed it is substantially easier to distill ODE models with straight trajectories. \cite{lee2023curvature,lee2024rfpp} also report combining RF models with higher-order solvers improves the trade-off between generation speed and quality.

% This is because OT ODEs minimize transport cost, and thus possess near-straight generative trajectories. Theoretically, a perfect OT ODE would be able to translate samples from one distribution to another with only a single velocity evaluation.

% However, it is unclear whether we can apply fast solvers to distilled models, as they do not generally learn an ODE between distributions.



==> sections/E_samples.tex <==

\section{Generated Samples}

\begin{figure}[H]
\centering
\includegraphics[width=0.8\linewidth]{figures/sample_nfe5_cifar10.jpg}
\caption{CIFAR10, $\NFE = 9$, $\FID = 2.34$.}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=0.8\linewidth]{figures/sample_nfe5_afhqv2.jpg}
\caption{$\NFE = 9$ samples on AFHQv2, $\FID = 2.45$.}
\end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/sample_nfe5_ffhq.jpg}
% \caption{$\NFE = 9$ samples on FFHQ, $\FID = 3.15$.}
% \end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=0.8\linewidth]{figures/sample_nfe5_imagenet.jpg}
\caption{$\NFE = 9$ samples on ImageNet, $\FID = 2.60$.}
\end{figure}

==> sections/ethics_reproducibility.tex <==
% \section*{Ethics and Reproducibility}

% \textbf{Ethics statement.}

% \textbf{Reproducibility.}

==> tables/ablation_tables.tex <==
\begin{table}[t]
\begin{center}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{$\bm{n}$} & \multirow{2}{*}{\textbf{Iter.}} & \multirow{2}{*}{\textbf{solver}} & \multirow{2}{*}{\textbf{disc.}} & \multicolumn{6}{c}{\textbf{Num. Func. Eval.}} \\
\cmidrule(lr){6-11}
& & & & & $1$ & $3$ & $5$ & $7$ & $9$ & $> 10$ \\
\cmidrule{1-11}
% EDM & 1 & $300k$ & Heun & & 386 & 468 & 320 & 100 & 38.4 & 1.97 (35) \\
% \cmidrule(lr){1-11}
% RF++   & 2 & $800k$ & -- & & 3.38 & 2.60 & 2.53 & 2.51 & 2.47 & 2.47 (16) \\
% Ours   & 2 & $200k$ & --  &  & 5.50 & 2.64 & 2.43 & 2.37 & 2.32 & -- \\
Ours   & 2 & $200k$ & Heun & Linear & 5.50 & 3.05 & 2.66 & 2.44 & 2.49 & -- \\
   &  &  &  & EDM & 5.50 & 79.9 & 51.8 & 18.7 & 4.13 & -- \\
   &  &  &  & Sigmoid & 5.50 & 2.64 & 2.43 & 2.37 & 2.32 & -- \\
\bottomrule
\end{tabular}}
\end{center}
\caption{$\FID_{50k}$ on CIFAR10, resolution $32 \times 32$.}
\label{tab:cifar10_fid}
\vspace{-3mm}
\end{table}


\begin{table}[t]
\begin{center}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{$\bm{n}$} & \multirow{2}{*}{\textbf{Iter.}} &  \multirow{2}{*}{\textbf{smp}} & \multicolumn{6}{c}{\textbf{Num. Func. Eval.}} \\
\cmidrule(lr){6-11}
& & & & & $1$ & $3$ & $5$ & $7$ & $9$ & $> 10$ \\
\cmidrule{1-11}
EDM & 1 & $300k$ & -- & \rom{2} & 290 & 467 & 345 & 143 & 57.1 & 2.39 (79) \\
\cmidrule(lr){1-11}
RF++   & 2 & $800k$ & -- & \rom{1} & 5.65 & 4.35 & 4.25 & 4.27 & 4.30 & 4.35 (16) \\
Ours   & 2 & $200k$ & -- & \rom{3} & 6.94 & 3.91 & 3.48 & 3.41 & 3.22 & -- \\
\bottomrule
\end{tabular}}
\end{center}
\caption{$\FID_{50k}$ on FFHQ, resolution $64 \times 64$.}
\label{tab:ffhq_fid}
\vspace{-3mm}
\end{table}
\jt{initial results here, will update with latest}
\jt{describe sampler, smp key}
